Explaining with Contrastive Phrasal Highlighting: A Case Study in Assisting Humans to Detect Translation Differences

Explainable NLP techniques primarily explain by answering "Which tokens in the input are responsible for this prediction?''. We argue that for NLP models that make predictions by comparing two input texts, it is more useful to explain by answering "What differences between the two inputs explain this prediction?''. We introduce a technique to generate contrastive highlights that explain the predictions of a semantic divergence model via phrase-alignment-guided erasure. We show that the resulting highlights match human rationales of cross-lingual semantic differences better than popular post-hoc saliency techniques and that they successfully help people detect fine-grained meaning differences in human translations and critical machine translation errors.

==> tables/application_grounded_examples.tex <==
{
\renewcommand{\arraystretch}{1.3}
\begin{table*}[!ht]
    \centering
    \scalebox{0.54}{
    \begin{tabular}{ll}
    \toprule[3pt]
    %\addlinespace[0.1cm]
    \\\multirow{3}{*}{\textbf{\textsc{en-pt}}}

    & Of course , I am confident that the eurozone 's \colorbox{yneon}{\hz \textcolor{darkgreen}{\textbf{ongoing}}} sovereign-debt crisis will be overcome , and that a more \colorbox{gneon}{\textcolor{airforceblue}{\textbf{fragmented}}} and ineffective Europe will emerge .\\
     & É claro que estou confiante que a crise da dívida soberana \colorbox{yneon}{\hz \textcolor{darkgreen}{\textbf{em curso , da}}} zona euro , será superada e que uma Europa mais \colorbox{gneon}{\textcolor{airforceblue}{\textbf{integrada}}} e eficaz surgirá .\\
    %
    & \textcolor{gray}{\textit{ (gloss) I am of course confident that the eurozone's \colorbox{blue3}{\hz ongoing} sovereign debt crisis will be overcome and that a more \colorbox{blue3}{integrated} and effective Europe will emerge.}}\\
    \addlinespace[0.2cm]

    \\\multirow{3}{*}{\textbf{\textsc{en-es}}}

    & Caretaker Prime Minister Julia Gillard claimed during the campaign of the 2010 \colorbox{yneon}{\hz \textcolor{darkgreen}{\textbf{state}}} election that she believed Australia should become a republic. \\% at the end of Queen Elizabeth II's reign.\\
    & Julia Gillard, primera ministra interina, sostuvo, durante la campaña de las elecciones \colorbox{yneon}{\hz \textcolor{darkgreen}{\textbf{federales}}} de 2010, que consideraba que Australia debería pasar a ser una república.\\ 
    & \textcolor{gray}{\textit{(gloss) Julia Gillard, acting Prime Minister, argued during the 2010 \colorbox{blue3}{\hz federal} election campaign that she believed Australia should become a republic.}}\\

    % LIME
        \\\multirow{3}{*}{\textbf{\textsc{en-fr}}}
    & Despite leaving the show in 1993, he retained \colorbox{yneon}{\textcolor{darkgreen}{\textbf{a senior role}}} and continued to receive tens of millions of dollars every season in royalties.\\
    & Malgré son départ de l'émission en 1993, il a conservé le \colorbox{yneon}{\textcolor{darkgreen}{\textbf{titre de producteur exécutif et}}} a continué à recevoir des dizaines de millions de dollars chaque saison en redevances.\\
    & \textcolor{gray}{\textit{(gloss) Despite leaving the show in 1993, he retained the \colorbox{blue3}{executive producer title and} continued to receive tens of millions of dollars each season in royalties.}}\\

    \\\toprule[3pt]

    \end{tabular}} 
    \caption{Examples of \hname highlights for \textsc{pt-en} (critical error detection) and \textsc{en-fr}, \textsc{en-es} (semantic divergence annotation).} 
  \label{tab:ced_examples}
\end{table*}
}


==> tables/intro_example.tex <==
\scalebox{0.5}{
\begin{tabular}{p{1.24\columnwidth}}
\\
\textsc{el} Τα μέτρα που εφαρμόστηκαν στην Ελλάδα 
\colorbox{darkgreen!15}{\makebox(40,5){\textcolor{darkgreen}{δέχθηκαν}}}
\colorbox{darkgreen!15}{\makebox(90,5){\textcolor{darkgreen}{πολλά θετικά σχόλια}}} \colorbox{amber!25}{\makebox(80,5){\textcolor{orange}{από τον ξένο τύπο}}}
που εξήρε την Ελλάδα 
για τον περιορισμό της εξάπλωσης της πανδημίας στη χώρα.\\
\addlinespace[0.5em]
\textsc{gloss} The measures put place in Greece \colorbox{darkgreen!15}{\makebox(60,5){\textcolor{darkgreen}{received many}}}
\colorbox{darkgreen!15}{\makebox(80,5){\textcolor{darkgreen}{positive comments}}}
\colorbox{amber!25}{\makebox(90,5){\textcolor{orange}{from the foreign press}}}
%\colorbox{amber!25}{\makebox(55,5){\textcolor{orange}{foreign press}}}
for having slowed the spread of the disease in the country.\\
\addlinespace[0.5em]
\textsc{en} The measures put in place in Greece 
\colorbox{magenta!25}{\makebox(60,5){\textcolor{red}{are among the}}}
\colorbox{magenta!15}{\makebox(160,5){\textcolor{red}{most proactive and strictest in Europe}}}
and have been \colorbox{darkgreen!15}{\makebox(35,5){\textcolor{darkgreen}{credited}}} \colorbox{amber!25}{\makebox(60,5){\textcolor{orange}{internationally}}} for having slowed the spread of the disease.\\
\\
\end{tabular}
}



\iffalse
\scalebox{0.5}{
\begin{tabular}{p{1.0\columnwidth}}
\\
\textsc{el} Τα μέτρα που εφαρμόστηκαν στην Ελλάδα 
\colorbox{darkgreen!15}{\makebox(140,5){\textcolor{darkgreen}{δέχθηκαν πολλά θετικά σχόλια}}} \colorbox{amber!25}{\makebox(50,5){\textcolor{orange}{από τον ξέ-}}}
\colorbox{amber!25}{\makebox(30,5){\textcolor{orange}{νο τύπο}}}
που εξήρε την Ελλάδα 
για τον περιορισμό της εξάπλωσης της πανδημίας στη χώρα.\\

\textsc{gloss} The measures put place in Greece \colorbox{darkgreen!15}{\makebox(150,5){\textcolor{darkgreen}{received many positive comments}}}
\colorbox{amber!25}{\makebox(40,5){\textcolor{orange}{from the}}}
\colorbox{amber!25}{\makebox(55,5){\textcolor{orange}{foreign press}}}
for having slowed the spread of the disease in the country.\\

\textsc{en} The measures put in place in Greece 
\colorbox{magenta!25}{\makebox(30,5){\textcolor{red}{are am-}}}
\colorbox{magenta!15}{\makebox(200,5){\textcolor{red}{ong the most proactive and strictest in Europe}}}
and have been \colorbox{darkgreen!15}{\makebox(35,5){\textcolor{darkgreen}{credited}}} \colorbox{amber!25}{\makebox(60,5){\textcolor{orange}{internationally}}} for having slowed the spread of the disease.\\
\\
\end{tabular}
}
\fi

==> tables/synthetic_annos.tex <==

\begin{table}[!ht]
    \centering
    \scalebox{0.4}{
    \begin{tabular}{ccc@{\hskip 0.5in}ccc}

\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
 \addlinespace[2em]
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
 \addlinespace[2em]
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\\

    \end{tabular}}
    \caption{Caption}
    \label{tab:ced_annotations}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!ht]
    \centering
    \scalebox{0.4}{
    \begin{tabular}{ccc@{\hskip 0.5in}ccc}

\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva \\
%
 \addlinespace[2em]
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
 \addlinespace[2em]
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive \\
%
\cellcolor{purple!10} \dive & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{purple!10} \dive & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva & \cellcolor{green!10} \equiva \\
%
\\

    \end{tabular}}
    \caption{Caption}
    \label{tab:ced_annotations}
\end{table}
